SparCE: Sparsity aware General Purpose Core Extensions to Accelerate Deep Neural Networks

Deep Neural Networks (DNNs) have emerged as the method of choice for solving a wide range of machine learning tasks. The enormous computational demands posed by DNNs have most commonly been addressed through the design of custom accelerators. However, these accelerators are prohibitive in many design scenarios (e.g., wearable devices and IoT sensors), due to stringent area/cost constraints. Accelerating DNNs on these low-power systems, comprising of mainly the general-purpose processor (GPP) cores, requires new approaches. We improve the performance of DNNs on GPPs by exploiting a key attribute of DNNs, i.e., sparsity. We propose Sparsity aware Core Extensions (SparCE)- a set of micro-architectural and ISA extensions that leverage sparsity and are minimally intrusive and low-overhead. We dynamically detect zero operands and skip a set of future instructions that use it. Our design ensures that the instructions to be skipped are prevented from even being fetched, as squashing instructions comes with a penalty. SparCE consists of 2 key micro-architectural enhancements- a Sparsity Register File (SpRF) that tracks zero registers and a Sparsity aware Skip Address (SASA) table that indicates instructions to be skipped. When an instruction is fetched, SparCE dynamically pre-identifies whether the following instruction(s) can be skipped and appropriately modifies the program counter, thereby skipping the redundant instructions and improving performance. We model SparCE using the gem5 architectural simulator, and evaluate our approach on 6 image-recognition DNNs in the context of both training and inference using the Caffe framework. On a scalar microprocessor, SparCE achieves 19%-31% reduction in application-level. We also evaluate SparCE on a 4-way SIMD ARMv8 processor using the OpenBLAS library, and demonstrate that SparCE achieves 8%-15% reduction in the application-level execution time.

==> relatedwork.tex <==
\noindent
Prior research efforts that target improving the computational efficiency of DNNs can be grouped into the following broad classes.

\vspace{3pt}
\noindent \textbf{Software parallelization on multi-cores and GPUs.} A large number of previous efforts have been directed towards developing techniques for efficient parallelization of DNNs on multi-core servers and GPUs~\cite{Krizhevsky:2014, Iandola:2015, Dean:2012, Rhu:2016, Das:2016, Zlateski:2016, Nervana:2016}. However, the scalability of these techniques is often limited by synchronization and communication bottlenecks.

\vspace{3pt}
\noindent \textbf{Specialized accelerators.} Developing specialized hardware architectures has been an attractive approach to improve the computational efficiency of DNNs. These accelerators~\cite{Chen:2014,Chen:2014:1,Venkataramani:2017,Jouppi:2017,Majumdar:2012,Gokhale:2014,Farabet:2011,eyeriss,Chakradhar:2010, Reagen:2016, Eldridge:2015} utilize specialized processing cores, interconnect network and other hardware-software co-design methodologies to leverage the different forms of compute and data reuse patterns in DNNs.

\vspace{3pt}
\noindent \textbf{Approximate computing.} DNNs and the applications that use them are intrinsically resilient to errors in their underlying computations. Approximate computing techniques, such as low-precision implementations~\cite{Courbariaux:2015,Gupta:2015,Zhu:2016,Venkataramani:2014}, model compression~\cite{deepComp,Jaderberg:2014} and others~\cite{Seide:2014,Zhang:2015:1}, leverage this property to improve the computational efficiency of DNNs. 

\vspace{3pt}
\noindent \textbf{Post-CMOS technology.} Post-CMOS technologies such as memristors and spintronics have succeeded in realizing the computational primitives of DNNs through their intrinsic device characteristics. Implementations of small scale DNNs using memristor crossbar arrays~\cite{Liu:2015,Shafiee:2016} and spintronic devices~\cite{Ramasubramanian:2014} have demonstrated significant promise.

All the above efforts are complementary to \sagpp, as unlike above efforts, we attempt to leverage sparsity in the different DNN data-structures to improve efficiency on cost constrained embedded platforms comprising of mainly a GPP core.

\vspace{3pt}
\noindent \textbf{Exploiting sparsity.} Prior efforts that exploit sparsity to improve DNN efficiency can be grouped to two classes based on whether they exploit static sparsity or dynamic sparsity, as shown in Figure~\ref{fig:relwork}. Specialized sparse architectures that are capable of exploiting both static and dynamic sparsity incorporate a variety of compression techniques and zero-skipping schemes to reduce storage requirement and avoid redundant multiplications in accelerators~\cite{cnvlutin, eyeriss, eie, scnn, cambriconx, Park:2016}. 

On the other hand, software approaches that exploit weight sparsity on GPPs take advantage of sparse matrix libraries. These sparse libraries usually yield performance improvement only under extreme levels of sparsity ($>$95\%). Since DNNs naturally exhibit sparsity in the range of 40\%-70\%, a few research efforts force more weight sparsity into DNNs using sparse decomposition methods, \emph{etc.}~\cite{BLiu:2015,Wen:2016} or customize the pruning to match the underlying hardware organization~\cite{Yu:2017}. These invariably come at the cost of training overhead or loss of functional accuracy. In contrast, we propose micro-architectural extensions to GPPs that can exploit both dynamic and static sparsity while being effective even under intermediate levels. Thus, \sagpp~is able to exploit feature sparsity in several state-of-the-art dense DNN models as well as both feature and weight sparsity in existing pruned DNN models.    


%For example, Cnvlutin~\cite{cnvlutin} proposes techniques to avoid ineffectual multiplications associated with zero input feature values on the DaDianNao accelerator,  the Eyeriss~\cite{eyeriss} accelerator uses run-length encoding of zeros and gates the multiplier whenever it sees a zero input feature value, the EIE accelerator~\cite{eie} has in-built mechanisms of compressing the zero values and delivering only non-zero values of input features and weights of a fully connected layer, the SCNN accelerator~\cite{scnn} implements a data compression and dataflow technique for exploiting both feature and weight sparsity in convolutional layers, 

%In this section, we summarize the efforts in each of these classes and highlight the unique features of our work. from several important domains like recognition, mining, synthesis, search and vision, demonstrate an intrinsic error resiliency that allows them to produce outputs of acceptable quality even when some of the underlying computations are performed in an approximate or imprecise manner. \sagpp~falls directly into this class of efforts and we delve into more details of the other approaches exploiting sparsity to improve the efficiency of DNNs. For example, sparse convolutional neural network models can be developed through sparse decomposition and executed using specialized sparse matrix multiplication routines~\cite{BLiu:2015}. Other techniques for structured sparsity can also be used to develop sparse models~\cite{Wen:2016}.


